Nek5000/RS Performance on Advanced GPU Architectures

We demonstrate NekRS performance results on various advanced GPU architectures. NekRS is a GPU-accelerated version of Nek5000 that targets high performance on exascale platforms. It is being developed in DOE's Center of Efficient Exascale Discretizations, which is one of the co-design centers under the Exascale Computing Project. In this paper, we consider Frontier, Crusher, Spock, Polaris, Perlmutter, ThetaGPU, and Summit. Simulations are performed with 17x17 rod-bundle geometries from small modular reactor applications. We discuss strong-scaling performance and analysis.

==> header.tex <==


\newcommand{\Natural}{\mbox{${\bf N}$}}
\newcommand{\Integer}{\mbox{${\bf Z}$}}
\newcommand{\Real}{\mbox{${\bf R}$}}
\newcommand{\Complex}{\mbox{${\bf C}$}}

\newcommand{\Eps}{\varepsilon}
\newcommand{\Alpha}{A}
\newcommand{\Beta}{B}
\newcommand{\Epsilon}{E}
\newcommand{\Zeta}{Z}
\newcommand{\Eta}{H}
\newcommand{\Iota}{I}
\newcommand{\Kappa}{K}
\newcommand{\Mu}{M}
\newcommand{\Nu}{N}
\newcommand{\omicron}{o}
\newcommand{\Omicron}{O}
\newcommand{\Rho}{R}
\newcommand{\Tau}{T}
\newcommand{\Chi}{X}

\newcommand{\Sfrac}[2]{\mbox{\small$\frac{#1}{#2}$\normalsize}}
\newcommand{\Half}{\Sfrac{1}{2}}
\newcommand{\Vect}[1]{{\bf #1}}
\newcommand{\Grad}[1]{\nabla #1}
\newcommand{\Gradp}[1]{\nabla' #1}
\newcommand{\Gradx}[1]{\nabla_x #1}
\newcommand{\Gradxp}[1]{\nabla_{x'} #1}
\newcommand{\GradAlphap}[1]{\nabla_{\alpha}' #1}
\newcommand{\Div}[1]{\text{div}\left[#1\right]}
\newcommand{\Divp}[1]{\text{div}'\left[#1\right]}
\newcommand{\Divx}[1]{\text{div}_x \left[#1\right]}
\newcommand{\Divxp}[1]{\text{div}_{x'} \left[#1\right]}
\newcommand{\Curl}[1]{\text{curl}[#1]}
\newcommand{\Laplacian}[1]{\Delta #1}
\newcommand{\Laplacianp}[1]{\Delta' #1}
\newcommand{\Laplacianx}[1]{\Delta_x #1}
\newcommand{\Laplacianxp}[1]{\Delta_{x'} #1}
\newcommand{\Biharmonic}[1]{\Delta^2 #1}
\newcommand{\FT}[1]{{\cal F} \left\{ #1 \right\}}
\newcommand{\FTI}[1]{{\cal F}^{-1} \left\{ #1 \right\}}
\newcommand{\Variation}[2]{\delta_{#2} #1}

\newcommand{\Norm}[2]{\left\|#1\right\|_{#2}}
\newcommand{\LeftNorm}[1]{\left\|#1\right.}
\newcommand{\RightNorm}[2]{\left.#1\right\|_{#2}}
\newcommand{\SupNorm}[1]{\left|#1\right|_{L^{\infty}}}
\newcommand{\HolderNorm}[2]{\left|#1\right|_{C^{#2}}}
\newcommand{\SobNorm}[2]{\left\|#1\right\|_{H^{#2}}}

\newcommand{\InnerProd}[2]{\left\langle#1,#2\right\rangle}
\newcommand{\DotProd}[2]{\left\langle#1,#2\right\rangle}
\newcommand{\Abs}[1]{\left|#1\right|}
\newcommand{\Mod}[1]{\left|#1\right|}
\newcommand{\Angle}[1]{\langle #1 \rangle}
\newcommand{\RealPart}[1]{\text{Re\{}#1\text{\}}}
\newcommand{\ImagPart}[1]{\text{Im\{}#1\text{\}}}
\newcommand{\Null}[1]{\mbox{${\cal N}$}(#1)}
\newcommand{\Ran}[1]{\text{ran}(#1)}
\newcommand{\Ker}[1]{\text{ker}(#1)}
\newcommand{\Dim}[1]{\text{dim}(#1)}
\newcommand{\Rank}[1]{\text{rank}(#1)}
\newcommand{\Det}[1]{\mbox{det} #1}
\newcommand{\Span}[1]{\text{span}(#1)}
\newcommand{\sgn}{\text{sgn}}

\newcommand{\sech}{\mbox{$\mathrm{sech}$}}
\newcommand{\csch}{\mbox{$\mathrm{csch}$}}

\newcommand{\Intersect}{\cap}
\newcommand{\Union}{\cup}

\newcommand{\dftl}[1]{\; d#1}
\newcommand{\dV}{\dftl{V}}
\newcommand{\dS}{\dftl{S}}
\newcommand{\dx}{\dftl{x}}
\newcommand{\dy}{\dftl{y}}
\newcommand{\dz}{\dftl{z}}
\newcommand{\ds}{\dftl{s}}
\newcommand{\dt}{\dftl{t}}
\newcommand{\du}{\dftl{u}}
\newcommand{\dsigma}{\dftl{\sigma}}
\newcommand{\dxi}{\dftl{\xi}}

\newcommand{\BigOh}[1]{\mathcal{O}(#1)}
\newcommand{\LittleOh}[1]{\mathcal{o}(#1)}

\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cJ}{\mathcal{J}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cZ}{\mathcal{Z}}

\newcommand{\px}{\partial_x}
\newcommand{\py}{\partial_y}
\newcommand{\pz}{\partial_z}
\newcommand{\pt}{\partial_t}

\newcommand{\sumn}{\sum_{n=0}^{\infty}}
\newcommand{\sumno}{\sum_{n=1}^{\infty}}
\newcommand{\sumk}{\sum_{k=-\infty}^{\infty}}
\newcommand{\sump}{\sum_{p=-\infty}^{\infty}}

\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\bes}{\begin{equation*}}
\newcommand{\ees}{\end{equation*}}
\newcommand{\bse}{\begin{subequations}}
\newcommand{\ese}{\end{subequations}}

\newcommand{\Schrodinger}{Schr\"odinger}
\newcommand{\Holder}{H\"older}
\newcommand{\Calderon}{Calder\'{o}n}
\newcommand{\Pade}{Pad\'{e}}

\newcommand{\Question}[1]{\fbox{ {\bf Q: #1} }}
\newcommand{\Corrected}[1]
{\noindent \rule{\linewidth}{.75mm} \\ {\bf CORRECTED UP TO HERE (#1)} \\ \rule{\linewidth}{.75mm}}

\newcommand{\EE}{\mathbf{E}}
\newcommand{\EEt}{\mathbf{\tilde{E}}}
\newcommand{\Ex}{E^1}
\newcommand{\Ey}{E^2}
\newcommand{\Ez}{E^3}
\newcommand{\Ei}{\mathbf{E^i}}
\newcommand{\Eix}{E^{i,1}}
\newcommand{\Eiy}{E^{i,2}}
\newcommand{\Eiz}{E^{i,3}}
\newcommand{\Eit}{\mathbf{\tilde{E}^i}}

\newcommand{\Ep}{\mathbf{E^{+}}}
\newcommand{\Epx}{E^{+,1}}
\newcommand{\Epy}{E^{+,2}}
\newcommand{\Epz}{E^{+,3}}
\newcommand{\Em}{\mathbf{E^{-}}}
\newcommand{\Emx}{E^{-,1}}
\newcommand{\Emy}{E^{-,2}}
\newcommand{\Emz}{E^{-,3}}
\newcommand{\Epm}{\mathbf{E^{\pm}}}
\newcommand{\Epmx}{E^{\pm,1}}
\newcommand{\Epmy}{E^{\pm,2}}
\newcommand{\Epmz}{E^{\pm,3}}

\newcommand{\HH}{\mathbf{H}}
\newcommand{\HHt}{\mathbf{\tilde{H}}}
\newcommand{\Hx}{H^1}
\newcommand{\Hy}{H^2}
\newcommand{\Hz}{H^3}
\newcommand{\Hi}{\mathbf{H^i}}
\newcommand{\Hit}{\mathbf{\tilde{H}^i}}

\newcommand{\Hp}{\mathbf{H^{+}}}
\newcommand{\Hpx}{H^{+,1}}
\newcommand{\Hpy}{H^{+,2}}
\newcommand{\Hpz}{H^{+,3}}
\newcommand{\Hm}{\mathbf{H^{-}}}
\newcommand{\Hmx}{H^{-,1}}
\newcommand{\Hmy}{H^{-,2}}
\newcommand{\Hmz}{H^{-,3}}
\newcommand{\Hpm}{\mathbf{H^{\pm}}}
\newcommand{\Hpmx}{H^{\pm,1}}
\newcommand{\Hpmy}{H^{\pm,2}}
\newcommand{\Hpmz}{H^{\pm,3}}

\newcommand{\JJ}{\mathbf{J}}
\newcommand{\Jx}{J^1}
\newcommand{\Jy}{J^2}
\newcommand{\Jz}{J^3}
\newcommand{\JJt}{\mathbf{\tilde{J}}}

\newcommand{\AVec}{\mathbf{A}}
\newcommand{\Ax}{A^1}
\newcommand{\Ay}{A^2}
\newcommand{\Az}{A^3}
\newcommand{\BVec}{\mathbf{B}}
\newcommand{\Bx}{B^1}
\newcommand{\By}{B^2}
\newcommand{\Bz}{B^3}
\newcommand{\kVec}{\mathbf{k}}
\newcommand{\xVec}{\mathbf{x}}
\newcommand{\eeg}{e^{i(\alpha x + \beta y - \gamma g(x,y))}}
\newcommand{\DD}{\mathbf{D}}

\newcommand{\nn}{\mathbf{n}}
\newcommand{\NN}{\mathbf{N}}

\newcommand{\kp}{k^{+}}
\newcommand{\km}{k^{-}}
\newcommand{\kpm}{k^{\pm}}
\newcommand{\gammap}{\gamma^{+}}
\newcommand{\gammam}{\gamma^{-}}
\newcommand{\gammapm}{\gamma^{\pm}}
\newcommand{\Upm}{U^{\pm}}

\newcommand{\hOm}{{\hat\Omega}}
\newcommand{\Om}{\Omega}
\newcommand{\Omt}{{\Omega (t)}}
\newcommand{\vv}{\mathbf{v}}
\newcommand{\vx}{v^1}
\newcommand{\vy}{v^2}
\newcommand{\vz}{v^3}
\newcommand{\cc}{\mathbf{c}}
\newcommand{\rr}{\mathbf{r}}
\newcommand{\bXi}{\mathbf{\xi}}
\newcommand{\xx}{\mathbf{x}}
\newcommand{\xX}{\mathbf{X}}
\newcommand{\bA}{\mathbf{A}}
\newcommand{\bB}{\mathbf{B}}
\newcommand{\uu}{\mathbf{u}}
\newcommand{\ww}{\mathbf{w}}
\newcommand{\tu}{\tilde{u}}
\newcommand{\tuu}{\tilde{\mathbf{u}}}
\newcommand{\tww}{\tilde{\mathbf{w}}}
\newcommand{\ux}{u^1}
\newcommand{\uy}{u^2}
\newcommand{\uz}{u^3}




==> pf.tex <==


%begin      p. fischer
\def\ds{\displaystyle}
\def\d{\partial}
\def\dO{\partial \Omega}
\def\epsm{\epsilon_{\mbox{mach}}}
\def\Ob{\bar \Omega}
\def\dOt{\tilde {\partial \Omega}}
\def\spn{ {\textstyle span} \{ }
\def\ee{{\hat {\underline e}}}
\def\uxh{{\hat {\underline x}}}
\def\eq{ \; = \; }
%\def\eqq{ \, \equiv \, }
\def\eqq{ \, := \, }
% \def\es{ \, = \, }
\def\es{ = }
\def\ea{ \; & = & \; }
\def\sp{ \; + \; }
\def\sm{ \; - \; }
\def\ds{ \Delta s }
\def\dt{ \Delta t }
\def\dx{ \Delta x }
\def\dy{ \Delta y }
\def\XX{\raisebox{0.3ex}{$\chi$}}
\def\cW{{\cal W}}
\def\cK{{\cal K}}
\def\cL{{\cal L}}
\def\cA{{\cal A}}
\def\cB{{\cal B}}
\def\cH{{\cal H}}
\def\cI{{\bf I}}
\def\cJ{{\cal J}}
\def\cM{{\cal M}}
\def\cN{{\cal N}}
\def\No{{N_o}}
\def\cR{{\cal R}}
\def\scriptO{{{\it O}\kern -.42em {\it `}\kern + .20em}}
\def\RR{{{\rm l}\kern - .15em {\rm R} }}
\def\PP{{{\rm l}\kern - .15em {\rm P} }}
%\def\L2{{{\cal L}^2}}
%\def\H1{{{\cal H}^1}}
%\def\L2{{{\bf L}^2}}
%\def\H1{{{\bf H}^1}}
\def\L2{{{\sf L}^2}}
\def\H1{{{\sf H}^1}}
\def\PN2{{\PP_{N}-\PP_{N-2}}}
\def\PNN{{\PP_{N}-\PP_{N}}}
\def\PNK{{\PP_{N,K}(\Omega)}}
\def\complex{{{\rm C} \kern - .53em {\rm l} \kern + .38em}}
\def\eop{\hbox{\vrule width 6pt height 6pt depth 0pt}}

\def\am{{ | \lambda_{\max} |}}
\def\a1{{ | \lambda_{\min} |}}
\def\lm{{   \lambda_{\max}  }}
\def\l1{{   \lambda_{\min}  }}
\def\bhu{{\hat   {\bf u}}}
\def\bhU{{\hat   {\bf {\underline u}}}}

\def\bff{{\bf f}}
\def\tp {{\tilde p}}
\def\tu {{\tilde u}}
\def\tx {{\tilde x}}
\def\btu{{\tilde {\bf u}}}
\def\bub{{\bar {\bf u}}}
\def\uet{{\tilde {\underline e}}}
\def\utU{{\underline {\tilde {\bf u}}}}
\def\uU{{{\underline {\bf u}}}}
\def\bhu{{\hat   {\bf u}}}
\def\bhn{{\hat   {\bf n}}}
\def\bhx{{\hat   {\bf x}}}
\def\bhy{{\hat   {\bf y}}}
\def\bhz{{\hat   {\bf z}}}
\def\ugt{{\tilde {\underline g}}}
\def\uut{{\tilde {\underline u}}}
\def\uxt{{\tilde {\underline x}}}
\def\ubt{{\tilde {\underline b}}}
\def\ubx{{\tilde {\underline x}}}
\def\bue{{\underline {\bf e}}}
\def\bur{{\underline {\bf r}}}
\def\bu0{{\underline {\bf 0}}}
\def\buu{{\underline {\bf u}}}
\def\buf{{\underline {\bf f}}}
\def\br{{\bf r}}
\def\bz{{\bf z}}
\def\bu{{\bf u}}
\def\bs{{\bf s}}
\def\bg{{\bf g}}
\def\bv{{\bf v}}
\def\bw{{\bf w}}
\def\bx{{\bf x}}
\def\bA{{\bf A}}
\def\bN{{\bf N}}
\def\bE{{\bf E}}
\def\bH{{\bf H}}
\def\bS{{\bf s}}
\def\Ab{{\bar A}}
\def\Hb{{\bar H}}
\def\nb{{\bar n}}
\def\bB{{\bf B}}
\def\bD{{\bf D}}
\def\bH{{\bf H}}
\def\bI{{\bf I}}
\def\bQ{{\bf Q}}

\def\Rt{{\tilde R}}
\def\At{{\tilde A}}
\def\Bt{{\tilde B}}
\def\Bb{{\bar B}}
\def\Dt{{\tilde D}}
\def\It{{\tilde I}}
\def\Ut{{\tilde U}}
\def\ft{{\tilde f}}
\def\ct{{\tilde c}}
\def\wN{{\widetilde N}}
\def\ch{{\hat c}}
\def\uft{{\tilde {\underline f}}}

\def\Ah{{\hat A}}
\def\wh{{\hat \omega}}
\def\wb{{\bar \omega}}
\def\Fh{{\hat F}}
\def\fh{{\hat f}}
\def\ih{{{\hat \imath}}}
\def\jh{{{\hat \jmath}}}
\def\Bh{{\hat B}}
\def\Dh{{\hat D}}
\def\Eh{{\hat E}}
\def\Qh{{\hat Q}}
\def\Oh{{\hat \Omega}}
\def\Ot{{\tilde \Omega}}
\def\Ok{{\Omega^k}}
\def\Rh{{\hat R}}
\def\hu{{\hat u}}
\def\hv{{\hat v}}
\def\yh{{\hat y}}
\def\ufh{{\underline {\hat f}}}
\def\uyh{{\underline {\hat y}}}

\def\ulambda{{\underline \lambda}}
\def\ua{{\underline a}}
\def\ub{{\underline b}}
\def\uc{{\underline c}}
\def\ud{{\underline d}}
\def\ue{{\underline e}}
\def\uf{{\underline f}}
\def\ug{{\underline g}}
\def\uh{{\underline h}}
\def\ui{{\underline i}}
\def\uj{{\underline j}}
\def\uk{{\underline k}}
\def\ul{{\underline l}}
\def\um{{\underline m}}
\def\un{{\underline n}}
\def\uo{{\underline o}}
\def\up{{\underline p}}
\def\uq{{\underline q}}
\def\ur{{\underline r}}
\def\us{{\underline s}}
\def\ut{{\underline t}}
\def\uu{{\underline u}}
\def\uv{{\underline v}}
\def\uw{{\underline w}}
\def\ux{{\underline x}}
\def\vx{{\vec x}}
\def\uy{{\underline y}}
\def\uz{{\underline z}}
\def\u0{{\underline 0}}
\def\uK{{\underline K}}

\def\uxb{{\bar {\underline x}}}
\def\uub{{\bar {\underline u}}}
\def\uvb{{\bar {\underline v}}}
\def\ufb{{\bar {\underline f}}}
\def\utb{{\tilde {\underline u}}}
\def\udp{{\underline {\Delta p}}}
\def\utphi{{\tilde {\underline \Phi}}}
\def\uphi{{{\underline \Phi}}}

\def\inn{ {\textstyle \;  \; {\rm in} \;  }}
\def\onn{ {\textstyle \;  \; {\rm on} \;  }}
\def\for{ {\textstyle \;  \; {\rm for} \;  }}

\newcommand{\pp}[2]{\frac{\partial #1}{\partial #2} }
\newcommand{\dd}[2]{\frac{d #1}{d #2} }
\newcommand{\de}[2]{\frac{\delta #1}{\delta #2} }


%end        p. fischer


==> preambl.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Geometry 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\usepackage{geometry}
%\geometry{left   = 1.0in,
%          right  = 1.0in,
%          top    = 1.0in,
%          bottom = 1.0in}

\usepackage{moreverb,url}
\usepackage{amssymb,amsmath,amsfonts}
\usepackage{graphicx}
\usepackage{rotating}

\usepackage{setspace}
\usepackage{lipsum}
%\newcommand{\verbatimfont}[1]{\renewcommand{\verbatim@font}{\ttfamily#1}}
\usepackage{epstopdf}
\usepackage{alltt}
\usepackage{color}
\usepackage{multirow}
\usepackage{listings}

\usepackage{fancyvrb}
\fvset{fontsize=\scriptsize}
%\fvset{fontsize=\footnotesize}
\RecustomVerbatimEnvironment{verbatim}{Verbatim}{}

\usepackage{floatrow}
\floatsetup[table]{capposition=top}
\usepackage{algpseudocode,algorithm,algorithmicx}
%\usepackage{algcompatible}
\usepackage{todonotes}

\usepackage[per-mode=symbol]{siunitx}
\usepackage{pgfplots}
%\pgfplotsset{compat=1.17}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Formats
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\usepackage{subfigure,pgfplots,epsf,graphicx,color}
\usepackage{amsmath,amsfonts,amsthm,multirow}

\usepackage{comment}
\usepackage{rotating}
\usepackage{tabularx}
\usepackage{float}

\usepackage{pdfpages}
\usepackage{afterpage}
\usepackage{wrapfig}
\usepackage{microtype}
\usepackage{fullpage}
\usepackage{bm} 
\usepackage{caption} 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Colors
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\usepackage[colorlinks=true]{hyperref}
\hypersetup{
  colorlinks  = true, %Colours links instead of ugly boxes
  urlcolor    = blue, %Colour for external hyperlinks
  linkcolor   = blue, %Colour of internal links
  citecolor   = blue, %Colour of citations
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% epstopdf
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\newif\ifpdf
%\ifx\pdfoutput\undefined
%   \pdffalse
%\else
%   \pdfoutput=1
%   \pdftrue
%\fi
%\ifpdf
%   \usepackage[update,prepend]{epstopdf}
%   \DeclareGraphicsRule{.eps}{pdf}{.pdf}{`epstopdf #1}
%   \pdfcompresslevel=9
%\fi

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Style 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\usepackage{authblk}
\usepackage{chngcntr}
\usepackage{mcs_pack}

\DeclareGraphicsExtensions{.gif,.png,.jpg,.pdf,.tiff,.eps}	

\def\baselinestretch{1.0}
\textwidth 6.5in
\textheight 8.50in
\topmargin -0.15in
\parskip   0.05in
\oddsidemargin 0.0in
\parindent 5ex
\renewcommand{\topfraction}{.95}
\renewcommand{\bottomfraction}{.95}
\renewcommand{\textfraction}{.05}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\VI{\bold{v}}
%\newcommand{\projectname}{SHARP Thermal-Hydraulics}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




